Can Federated Learning Safeguard Private Data in LLM Training? Vulnerabilities, Attacks, and Defense Evaluation

Fine-tuning large language models (LLMs) with local data is a widely adopted approach for organizations seeking to adapt LLMs to their specific domains. Given the shared characteristics in data across different organizations, the idea of collaboratively fine-tuning an LLM using data from multiple sources presents an appealing opportunity. However, organizations are often reluctant to share local data, making centralized fine-tuning impractical. Federated learning (FL), a privacy-preserving framework, enables clients to retain local data while sharing only model parameters for collaborative training, offering a potential solution. While fine-tuning LLMs on centralized datasets risks data leakage through next-token prediction, the iterative aggregation process in FL results in a global model that encapsulates generalized knowledge, which some believe protects client privacy. In this paper, however, we present contradictory findings through extensive experiments. We show that attackers can still extract training data from the global model, even using straightforward generation methods, with leakage increasing as the model size grows. Moreover, we introduce an enhanced attack strategy tailored to FL, which tracks global model updates during training to intensify privacy leakage. To mitigate these risks, we evaluate privacy-preserving techniques in FL, including differential privacy, regularization-constrained updates and adopting LLMs with safety alignment. Our results provide valuable insights and practical guidelines for reducing privacy risks when training LLMs with FL.

==> sections/abstract_orig.tex <==
Fine-tuning large language models (LLMs) with local data is a widely adopted practice among organizations aiming to tailor LLMs to their specific domains. Given the potential similarities in data across different organizations, the idea of collaboratively fine-tuning an LLM using data from multiple organizations presents an intriguing opportunity. However, a challenge arises: organizations are often unwilling to share their local data during the fine-tuning process, thus makes centralized fine-tuning, i.e. the LLM is trained on data collected from multiple organizations, unacceptable in many scenarios.
% Autoregressive large language models (LLMs) have achieved remarkable success across diverse tasks, but training them requires substantial data, which is often constrained by privacy concerns.
Federated learning (FL), a privacy-preserving framework that 
[enables multiple clients to collaboratively train a model without exposing their local data,
/enables multiple clients to retain their data locally while sharing only model parameters to collaboratively train a global model,]
emerges as a natural solution. Furthermore, models fine-tuned through FL appear to offer an additional advantage. While fine-tuning LLMs on a centralized dataset inherently risks data leakage due to the next-token prediction mechanism, the global model in FL is derived from iterative aggregation across multiple clients. This process results in a model that encapsulates generalized, non-specific knowledge, leading some researchers to believe that the global model inherently safeguards the privacy of individual clients.
% Federated learning (FL) offers a solution by enabling data owners to retain their data locally while sharing only model parameters, thereby facilitating the collaborative training of a powerful global model.
In this paper, however, we present contradictory findings through extensive experiments. We demonstrate that attackers can still extract training data from the global model using straightforward generation techniques, and the extent of leakage increases with model size. Furthermore, we propose an enhanced attack strategy specifically designed for FL, which leverages global model updates during training to exacerbate privacy leakage.
% However, \textit{can FL truly protect training data from leakage during LLM training?}
% The data privacy protection in FL relies on two necessary prerequisites: first, that recovering training data from model parameters is difficult, and second, that the shared global model contains only general, non-specific knowledge.
% While these prerequisites are satisfied in traditional tasks, they may not hold for training LLMs.
% The nature of next-token prediction in LLMs makes it more likely that data can be recovered from models. Additionally, the large parameter volume of LLMs increases the risk of storing private information, posing significant threats to the privacy protection capabilities of FL.
% To investigate this, we conduct experiments across various scenarios, showing that attackers can extract training data from global model with a simple generation method, and the severity increases as the model size grows.
% We also propose an enhanced attack strategy that tracks global model updates to amplify the privacy leakage.
To mitigate these risks, we evaluate privacy-preserving techniques in FL, including differential privacy and regularization-constrained updates. Our results provide critical insights and practical guidelines for reducing privacy risks when training LLMs using FL.
% To address these threats, we assess privacy-preserving techniques in FL, such as differential privacy and regularization-constrained updates.
% Our findings provide in-depth insights and practical guidelines for mitigating privacy risks when training LLMs with FL.


==> sections/discussion.tex <==
% Discuss: 1) guidelines to train LLMs in FL; 2) Anything interesting that is worthwhile to be discussed; 3) broader impacts of this paper
Our findings challenge the assumption that Federated Learning (FL) inherently prevents privacy leakage in large language model (LLM) training. While FL avoids direct data sharing, the generative nature of LLMs and FL's iterative aggregation still pose significant privacy risks. Techniques like differential privacy (DP) and KL-divergence regularization can mitigate these risks, but they come with a trade-off in model performance, especially in terms of slower convergence.

Furthermore, We propose that alternative fine-tuning methods, such as Differential Privacy Optimization (DPO) and Reinforcement Learning from Human Feedback (RLHF), which align model preferences rather than memorizing specific training data, potentially reducing privacy risks. We recommend that federated training frameworks explore these approaches to balance privacy and model performance.

In addition to our main experiments, we also conducted additional studies, such as perturbing the input data to simulate scenarios with uncertain or partial information. The results of these experiments, which are detailed in Appendix~\ref{appendix:disturbed}.

This paper highlights the need for more effective privacy-preserving techniques in federated LLM training. Future work should focus on solutions that protect privacy while maintaining the performance benefits of large models.
